Metalearning with Very Few Samples Per Task

Metalearning and multitask learning are two frameworks for solving a group of related learning tasks more efficiently than we could hope to solve each of the individual tasks on their own. In multitask learning, we are given a fixed set of related learning tasks and need to output one accurate model per task, whereas in metalearning we are given tasks that are drawn i.i.d. from a metadistribution and need to output some common information that can be easily specialized to new tasks from the metadistribution. We consider a binary classification setting where tasks are related by a shared representation, that is, every task $P$ can be solved by a classifier of the form $f_{P} \circ h$ where $h \in H$ is a map from features to a representation space that is shared across tasks, and $f_{P} \in F$ is a task-specific classifier from the representation space to labels. The main question we ask is how much data do we need to metalearn a good representation? Here, the amount of data is measured in terms of the number of tasks $t$ that we need to see and the number of samples $n$ per task. We focus on the regime where $n$ is extremely small. Our main result shows that, in a distribution-free setting where the feature vectors are in $\mathbb{R}^d$, the representation is a linear map from $\mathbb{R}^d \to \mathbb{R}^k$, and the task-specific classifiers are halfspaces in $\mathbb{R}^k$, we can metalearn a representation with error $\varepsilon$ using $n = k+2$ samples per task, and $d \cdot (1/\varepsilon)^{O(k)}$ tasks. Learning with so few samples per task is remarkable because metalearning would be impossible with $k+1$ samples per task, and because we cannot even hope to learn an accurate task-specific classifier with $k+2$ samples per task. Our work also yields a characterization of distribution-free multitask learning and reductions between meta and multitask learning.

==> img/fig_new_dataset.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,236); %set diagram left start at 0, and has height of 236

%Rounded Rect [id:dp4686430581840396] 
\draw  [line width=1.5]  (16,97.4) .. controls (16,87.79) and (23.79,80) .. (33.4,80) -- (87.6,80) .. controls (97.21,80) and (105,87.79) .. (105,97.4) -- (105,149.6) .. controls (105,159.21) and (97.21,167) .. (87.6,167) -- (33.4,167) .. controls (23.79,167) and (16,159.21) .. (16,149.6) -- cycle ;

%Straight Lines [id:da3750788988193219] 
\draw [line width=1.5]    (112,122) -- (166,122) ;
\draw [shift={(169,122)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Rounded Rect [id:dp4435815186381684] 
\draw  [line width=1.5]  (175,97.4) .. controls (175,87.79) and (182.79,80) .. (192.4,80) -- (246.6,80) .. controls (256.21,80) and (264,87.79) .. (264,97.4) -- (264,149.6) .. controls (264,159.21) and (256.21,167) .. (246.6,167) -- (192.4,167) .. controls (182.79,167) and (175,159.21) .. (175,149.6) -- cycle ;

%Rounded Rect [id:dp30983238640831057] 
\draw  [line width=1.5]  (341,61) .. controls (341,50.51) and (349.51,42) .. (360,42) -- (417,42) .. controls (427.49,42) and (436,50.51) .. (436,61) -- (436,181) .. controls (436,191.49) and (427.49,200) .. (417,200) -- (360,200) .. controls (349.51,200) and (341,191.49) .. (341,181) -- cycle ;

%Straight Lines [id:da5487016515746438] 
\draw [line width=1.5]    (272,121) -- (326,121) ;
\draw [shift={(329,121)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da06933398494211018] 
\draw [line width=1.5]    (446,119) -- (556,120) ;

%Rounded Rect [id:dp33255128078978835] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]  (8,62.4) .. controls (8,40.64) and (25.64,23) .. (47.4,23) -- (516.6,23) .. controls (538.36,23) and (556,40.64) .. (556,62.4) -- (556,180.6) .. controls (556,202.36) and (538.36,220) .. (516.6,220) -- (47.4,220) .. controls (25.64,220) and (8,202.36) .. (8,180.6) -- cycle ;
%Shape: Rectangle [id:dp9734065596391649] 
\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (45,4) -- (176,4) -- (176,44) -- (45,44) -- cycle ;

%Straight Lines [id:da5132714101876962] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (557,120) -- (581,120) ;
\draw [shift={(584,120)}, rotate = 180] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

% Text Node
\draw (27.23,103.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{46.94pt}\setlength\topsep{0pt}
\begin{center}
$\metadist$\\meta dist.
\end{center}

\end{minipage}};
% Text Node
\draw (185.23,103.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{49.27pt}\setlength\topsep{0pt}
\begin{center}
$\dist_i$\\task $\displaystyle i$ dist.
\end{center}

\end{minipage}};
% Text Node
\draw (58,14) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.25,0.46,0.02}{Distribution $\cD$}};
% Text Node
\draw (358.66,57) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{41.86pt}\setlength\topsep{0pt}
\begin{center}
Labeled \\samples\\$\displaystyle (\feat_{1}^{i},\, \lab_{1}^{i})$\\$\displaystyle (\feat_{2}^{i},\, \lab_{2}^{i})$\\$\displaystyle \vdots $\\$\displaystyle (\feat_{m}^{i},\,\lab_{m}^{i})$
\end{center}

\end{minipage}};
% Text Node
\draw (596,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\zeta _{i} \coloneqq ((\feat_1^i,\lab_1^i,\ldots, \feat_{\wit}^i, \lab_{\wit}^i), +1)$};
% Text Node
\draw (273,129) node [anchor=north west][inner sep=0.75pt]   [align=left] {m times};
% Text Node
\draw (274,96) node [anchor=north west][inner sep=0.75pt]   [align=left] {sample};
% Text Node
\draw (114,97) node [anchor=north west][inner sep=0.75pt]   [align=left] {sample};
% Text Node
\draw (449,127) node [anchor=north west][inner sep=0.75pt]   [align=left] {\& add label +1};
% Text Node
\draw (450,94) node [anchor=north west][inner sep=0.75pt]   [align=left] {Concatenate};


\end{tikzpicture}

==> meta_monotone.tex <==
We consider the composition of a linear representation function from $\datadim$ to $1$ dimension from class $\repclass_{\datadim,1} = \left\{\rep| \rep(\mathbf{\feat}) = \mathbf{b} \cdot \mathbf{\feat}, \mathbf{b} \in \R^{\datadim}\right\}$ with a monotone threshold from class 
$\perclass_{\textrm{mt}} = \left\{\per| \per(\map) = \textrm{sign}(\map - w), w \in \R \right\}$. 
\begin{thm}
    We can $(\eps,\delta)$-metalearn $(\repclass_{\datadim,1},\perclass_{\textrm{mt}})$ with $\users = O(\frac{d +\ln(1/\delta)}{\eps^2})$ tasks and $2$ samples per task in the realizable case.
\end{thm}
Every dataset with more than $2$ points that is not realizable by $\perclass_{\textrm{mt}}$ has a non-realizability witness of size $2$. To see this suppose all subsets of two points are realizable by $\perclass_{\textrm{mt}}$. This means that any points with positive labels are greater than points with negative points. In this case, there exists a monotone threshold that labels these points correctly. Thus, we have arrived at a contradiction.

The realizability predicate $\realp_\rep$ takes two labeled datapoints $(\mathbf{x}_1, y_1)$ and $(\mathbf{x}_2, y_2)$ from every task and returns $+1$ if $\rep$ orders them correctly. More formally, given an $\rep \in \repclass$ 
\[
\realp_\rep(\mathbf{x}_1, y_1, \mathbf{x}_2, y_2) = 
\begin{cases}
-1, & y_1 = +1, y_2 = -1 \textrm{ and } \rep(\mathbf{x}_1) < \rep(\mathbf{x}_2)\\
-1, & y_1 = -1, y_2 = +1 \textrm{ and } \rep(\mathbf{x}_1) > \rep(\mathbf{x}_2)\\
+1, & \textrm{otherwise.}
\end{cases}
\]
We can view $\realp_\rep$ as a classifier on datapoints of the form $(\mathbf{x}_1, y_1, \mathbf{x}_2, x_2)$. Since we work in the realizable setting, the correct representation will always order points correctly. Hence, we want to learn an $\rep \in \repclass_{d,1}$ which has low $\Pr[P \sim \metadist,(\mathbf{x}_1,y_1), (\mathbf{x}_2, y_2) \sim \dist^2]{\realp_\rep(\mathbf{x}_1, y_1, \mathbf{x}_2, y_2)=-1}$.
\begin{fact}
\label{fct:vc-hf}
\knote{citation?}
Let $\perclass = \{\per \mid \per(\mathbf{x}) = \sign (\mathbf{a}\cdot \mathbf{x}), \mathbf{a} \in \R^d\}$ be the class of $d$-dimensional halfspaces that pass through zero. Then $\VC(\perclass) = d$.
\end{fact}
\begin{lem}
\label{lem:vc_mt}
   The VC dimension of $\realpclass_{2, \perclass_{\textrm{mt}}, \repclass_{\datadim,1}}$ is 
   \[
   \VC(\realpclass_{2, \perclass_{\textrm{mt}}, \repclass_{\datadim,1}}) \leq 2d.
   \]
\end{lem}
\begin{proof}
    We can rewrite $\realp_\rep$ as 
    \[
    \realp_\rep(\mathbf{x}_1, y_1, \mathbf{x}_2, y_2) = \mathbbm{1}\{y_1=y_2\} + \mathbbm
    {1}\{y_1\neq y_2\}\textrm{sign}\left(\left(\mathbf{b}^T\| -\mathbf{b}^T\right)\cdot\begin{pmatrix}
        \mathbf{x}_1\\
        \mathbf{x}_2
    \end{pmatrix}\right).
    \]
    We notice that if in our dataset we have a datapoint with $y_1=y_2$, then this dataset cannot be shattered because the label for this datapoint can only be $+1$. Additionally, by \Cref{fct:vc-hf} the VC dimension of concept class $\cA_{\textrm{mt}}=\left\{a_h\mid a_h(\mathbf{x}_1, \mathbf{x}_2) = \textrm{sign}\left(\left(\mathbf{b}^T\| -\mathbf{b}^T\right)\cdot\begin{pmatrix}
        \mathbf{x}_1\\
        \mathbf{x}_2
    \end{pmatrix}\right)\right\}$ is at most $2d$, because $\cA_{\textrm{mt}}$ is a subclass of $2d$-dimensional halfspaces that pass through zero. The VC dimension of $\realpclass_{2, \perclass_{\textrm{mt}}, \repclass_{\datadim,1}}$ is also at most $2d$. This happens because if there exists a dataset $\left((\mathbf{x}_1^{(1)}, y_1^{(1)}, \mathbf{x}_2^{(1)}, y_2^{(1)}), \ldots, (\mathbf{x}_1^{(2d+1)}, y_1^{(2d+1)}, \mathbf{x}_2^{(2d+1)}, y_2^{(2d+1)})\right)$ of size $2d+1$ that can be shattered by $\realpclass_{2, \perclass_{\textrm{mt}}, \repclass_{\datadim,1}}$, then for all $i \in [2d+1]$ $y_1^{(i)} \neq y_2^{(i)}$ and $\left((\mathbf{x}_1^{(1)}, \mathbf{x}_2^{(1)}), \ldots, (\mathbf{x}_1^{(2d+1)}, \mathbf{x}_2^{(2d+1)})\right)$ can be shattered by $\cA_{\textrm{mt}}$. This is a contradiction because there is no dataset of size $2d+1$ that can be shattered by $\cA_{\textrm{mt}}$. 
\end{proof}
By \Cref{fact:pac-vc} and \Cref{lem:vc_mt} if we have $\users = O\left(\frac{d\ln(1/\eps)+\ln(1/\delta)}{\varepsilon^2}\right)$ tasks, each with two labeled datapoints $(\mathbf{x}_1^{(j)}, y_1^{(j)})$ and $(\mathbf{x}_2^{(j)}, y_2^{(j)})$, then by choosing  $\hat{\rep} \in \repclass_{d,1}$ which maximizes $\frac{1}{\users}\sum_{j \in [\users]}\realp_\rep(\mathbf{x}_1^{(j)}, y_1^{(j)}, \mathbf{x}_2^{(j)}, y_2^{(j)})$ we get that 
$\Pr[P \sim \metadist,(\mathbf{x}_1,y_1), (\mathbf{x}_2, y_2) \sim \dist^2]{\realp_{\hat{h}}(\mathbf{x}_1, y_1, \mathbf{x}_2, y_2)=-1} < \varepsilon^2$ with probability at least $1-\delta$ over the dataset.
\begin{fact}
\label{fact:auc}
\knote{citation?}
    Let $\textrm{TPR}(w) := \Pr[(\map,y)\sim \Task]{\map> w\mid y=+1}$ be the true positive rate of classifier $\textrm{sign}(\map-w)$ and $\textrm{FPR}(w):= \Pr[(\map,y)\sim P]{\map\geq w\mid y=-1}$ be the false positive rate of the same classifier. The plot of $\textrm{TPR}(w)$ against $\textrm{FPR}(w)$ for all values of $w \in \R$ is called the ROC curve. The area under the ROC curve, also known as AUC, is equal to $\Pr[\substack{(\map_1,y_1)\sim \dist\\ (\map_2,y_2)\sim \dist}]{\map_1>\map_2 \mid  y_1=+1, y_2=-1}$.
\end{fact}
\begin{lem}
\label{lem:mon-bnd}
Fix a distribution $\dist$ over $ \mapdom \times \{\pm 1\}$ and define
\begin{align*}
    \alpha_{r}&:= \Pr[(\map_1,y_1),(\map_2,y_2) \sim \Task^2]{(\map_1,y_1),(\map_2,y_2)\textrm{ is not realizable by }\perclass_{\textrm{mt}}}\\
    \alpha_{e}&:=\min_{w \in \R}\left\{ \Pr[(\textrm{\map},y)\sim P]{\textrm{sign}(\map-w)\neq y} \right \}
\end{align*}
Then
$ \alpha_r \geq \alpha_e^2$.
\end{lem}
\begin{proof}
Let $\rho= \Pr[(\map,y)\sim \Task]{y=1}$. We start by showing that
\begin{equation}
\label{eq:AUC}
\alpha_e^2 \leq 2\rho(1-\rho)(1-\Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \dist}]{\map_1>\map_2 \mid  y_1=+1, y_2=-1}).
\end{equation}
Let $\textrm{TPR}(w) := \Pr[(\map,y)\sim \Task]{\map> w\mid y=+1}$ be the true positive rate of classifier $\textrm{sign}(\map-w)$ and $\textrm{FPR}(w):= \Pr[(\map,y)\sim P]{\map\geq w\mid y=-1}$ be the false positive rate of the same classifier. Then,
\begin{align*}
\Pr[(\map,y)\sim \Task]{\textrm{sign}(\map-w)\neq y} 
&= \Pr[(\map,y)\sim \Task]{\map< w\mid y=+1}\rho + \Pr[(\map,y)\sim P]{\map\geq w\mid y=-1}(1-\rho)\\
&= (1-\textrm{TPR}(w))\rho+\textrm{FPR}(w)(1-\rho).
\end{align*}
The plot of $\textrm{TPR}(w)$ against $\textrm{FPR}(w)$ for all values of $w \in \R$ is called the ROC curve. In the same coordinate system, the points where line $(1-\textrm{TPR})\rho+\textrm{FPR}(1-\rho) = c$ intersects with the ROC curve have error $\Pr[(\map,y)\sim \Task]{\textrm{sign}(\map-w)\neq y}=c$. By \Cref{fact:auc} the area under the ROC curve is equal to $\Pr[\substack{(\map_1,y_1)\sim \dist\\ (\map_2,y_2)\sim \dist}]{\map_1>\map_2 \mid  y_1=+1, y_2=-1}$. Therefore, we can geometrically upper bound the AUC by the area under the isoerror line for error $\min_{w \in \R}\left\{ \Pr[(\map,y)\sim \Task]{\textrm{sign}(\map-w)\neq y} \right \}$ and line $\textrm{TPR} = 1$. This approach gives us the following bound
\begin{align*}
    \Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{\map_1>\map_2 \mid  y_1=+1, y_2=-1} \leq 1-\frac{\left(\min_{w \in \R}\left\{ \Pr[(\map,y)\sim \Task]{\textrm{sign}(\map-w) \neq y} \right \}\right)^2}{2\rho(1-\rho)}.
\end{align*}
We see that 
\[
\left(\min_{w \in \R}\left\{ \Pr[(\map,y)\sim \dist]{\textrm{sign}(\map-w)\neq y} \right \}\right)^2 \leq 2\rho (1-\rho)(1- \Pr[\substack{(\map_1,y_1)\sim \dist\\ (\map_2,y_2)\sim \dist}]{\map_1>\map_2 \mid  y_1=+1, y_2=-1}).
\]
Now, we connect the probability that two points drawn from distribution $\Task$ cannot be realized by $\perclass_{\textrm{mt}}$ with the probability that the features of a pair of a positive and a negative example that are drawn from $\Task$ are not ordered correctly. By the law of total probability, we have that 
\begin{align*}
    &\Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{(\map_1, y_1), (\map_2, y_2) \textrm{ is not realizable by}\perclass_{\textrm{mt}}}=\\
    &\sum_{i\in \bits} \sum_{j \in \bits}\Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{(\map_1, y_1), (\map_2, y_2) \textrm{ is not realizable by}\perclass_{\textrm{mt}}\mid y_1=i, y_2=j } \Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{y_1 = i, y_2=j} = \\
    &2\rho(1-\rho)\Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{\map_1\leq \map_2 \mid y_1=+1,y_2=-1} =\\
    &2\rho(1-\rho)(1-\Pr[\substack{(\map_1,y_1)\sim \Task\\ (\map_2,y_2)\sim \Task}]{\map_1> \map_2 \mid y_1=+1,y_2=-1}).
\end{align*}
Therefore, $\alpha_e^2 \leq \alpha_r$.
\end{proof}

For fixed representation $\rep \in \repclass_{\datadim,1}$ and distribution $\dist$ over $\featdom\times \{\pm 1\}$, \Cref{lem:mon-bnd} says that
\begin{align*}
    \min_{w \in \R}\left\{ \Pr[(\mathbf{\feat},y)\sim P]{\textrm{sign}(\rep(\mathbf{\feat})-w)\neq y} \right \} &\leq \sqrt{\Pr[\substack{(\mathbf{\feat}_1,y_1)\sim \Task\\ (\mathbf{\feat}_2,y_2)\sim \Task}]{(\rep(\mathbf{\feat}_1), y_1), (\rep(\mathbf{\feat}_2), y_2) \textrm{ is not realizable by}\perclass_{\textrm{mt}}}}\\
    & = \sqrt{\Pr[\substack{(\mathbf{\feat}_1,y_1)\sim \Task\\ (\mathbf{\feat}_2,y_2)\sim \Task}]{\realp_\rep(\mathbf{\feat}_1, \lab_1, \mathbf{\feat}_2, \lab_2) = -1}}.
\end{align*}
We now take the expectation over distribution $\metadist$ for representation $\hat{\rep}$
\begin{align*}
    \Exp_{P \sim Q}\left[\min_{w \in \R}\left\{ \Pr[(\textrm{x},y)\sim P]{\textrm{sign}(\hat{h}(\mathbf{x})-w)\neq y\}} \right \}\right] &\leq \Exp_{P \sim Q}\left[\sqrt{\Pr[\substack{(\mathbf{\feat}_1,y_1)\sim \Task\\ (\mathbf{\feat}_2,y_2)\sim \Task}]{\realp_{\hat{\rep}}(\mathbf{\feat}_1, \lab_1, \mathbf{\feat}_2, \lab_2) = -1}}\right]\\
    & \leq \sqrt{\Exp_{P \sim Q}\left[\Pr[\substack{(\mathbf{\feat}_1,y_1)\sim \Task\\ (\mathbf{\feat}_2,y_2)\sim \Task}]{\realp_{\hat{\rep}}(\mathbf{\feat}_1, \lab_1, \mathbf{\feat}_2, \lab_2) = -1}\right]},
\end{align*}
where the last step follows by Jensen's inequality. 

We conclude that with probability at least $1-\delta$ over the data (that we get by drawing a task $P$ from $Q$ and then two samples from $P$ for every task $j \in [\users]$)
\[
\Exp_{P \sim Q}\left[\min_{w \in \R}\left\{ \Pr[(\textrm{x},y)\sim P]{\textrm{sign}(\hat{h}(\mathbf{x})-w)\neq y\}} \right \}\right] \leq  \varepsilon.
\]

